Validation of TOI-1221 b: A warm sub-Neptune exhibiting TTVs around a Sun-like star

We present a validation of the long-period ($91.68278^{+0.00032}_{-0.00041}$ days) transiting sub-Neptune planet TOI-1221 b (TIC 349095149.01) around a Sun-like (m$_{\rm V}$=10.5) star. This is one of the few known exoplanets with period >50 days, and belongs to the even smaller subset of which have bright enough hosts for detailed spectroscopic follow-up. We combine TESS light curves and ground-based time-series photometry from PEST (0.3~m) and LCOGT (1.0~m) to analyze the transit signals and rule out nearby stars as potential false positive sources. High-contrast imaging from SOAR and Gemini/Zorro rule out nearby stellar contaminants. Reconnaissance spectroscopy from CHIRON sets a planetary scale upper mass limit on the transiting object (1.1 and 3.5 M$_{\rm Jup}$ at 1$\sigma$ and 3$\sigma$, respectively) and shows no sign of a spectroscopic binary companion. We determine a planetary radius of $R_{\rm p} = 2.91^{+0.13}_{-0.12} R_{\oplus}$, placing it in the sub-Neptune regime. With a stellar insolation of $S = 6.06^{+0.85}_{-0.77}\ S_{\oplus}$, we calculate a moderate equilibrium temperature of $T_{\rm eq} =$ 440 K, assuming no albedo and perfect heat redistribution. We find a false positive probability from TRICERATOPS of FPP $ = 0.0014 \pm 0.0003$ as well as other qualitative and quantitative evidence to support the statistical validation of TOI-1221 b. We find significant evidence (>$5\sigma$) of oscillatory transit timing variations, likely indicative of an additional non-transiting planet.

==> Old_false_positives_section_backup.tex <==

%%%% This is being saved as backup.
%%%%  I don't think it flows well, 
%%%%  so I'm restructuring it


The most likely false positives to occur in \tess{} observations involve transiting objects that are non-planetary in nature, either physically bound to the host, or simply situated in close sky-projected proximity.  When considering bound stellar companions, we can test for a number of typical indicators.  







%% Photometric FP rejection
In NEB false positive scenarios, transiting stellar companions of comparable size to their host star are prone to producing V-shaped transits or grazing geometries, both of which are argued against by the flat bottom and clear demarcations of ingress and egress seen in the light curves.
%
We also check the surrounding sky for potential NEB sources blended in the \tess\ aperture.  The PEST observation was able to clear all reasonably bright targets (within $\Delta$mag $\sim$ 7.5) in a $2\farcm5$ radius with the exception of the nearest neighbour, $13\farcs2$ away SWW, which was not cleanly resolved from the target.  


In this context, clearing a neighbour star means that the unblended light curves of these stars show significant non-detections of transit-like signals of a depth that would produce the observed flux drop in a blended {\it TESS} aperture.
%
Table~\ref{Tab:PEST_NEBs} shows the NEB potential for reasonably bright stars within $2\farcm5$ %\arcmin 
ruled out by the PEST observation.
%
The subsequent LCOGT-1m observations simultaneously detected a transit  on-target and was able to resolve and rule out an NEB signal on the $13\farcs2$ neighbour.  
%
With these small-telescope observations, we can conclude that sources from $2\farcm5$ down to $\sim$10\arcsec \ show no indication of NEB signals.  

We further probe tighter separations than was possible with the small ground-based telescope time series observations.  The {\it Gaia} DR3 catalogue \citep{Gaia_collaboration_2016,Gaia_DR3_2022} 
reports no sources within 12\arcsec, and so clears the area down to its resolving power of $\lesssim 1\arcsec$.
\cmc{(Mention Gaia completeness mag limits)}.
%% 
%% Gaia completeness
% \footnote{\url{https://gea.esac.esa.int/archive/documentation/GEDR3/Catalogue_consolidation/chap_cu9val/sec_cu9val_introduction/ssec_cu9val_intro_completeness.html}}
%%
For the region within 1\arcsec, we look at the acquired high contrast speckle imaging.  
%
The initial SOAR/HRCam and subsequent Gemini-S/Zorro images clear the surrounding sky of sources (at a 5$\sigma$ level) down to $\Delta$mag of 5.2 at $0\farcs1$ separation 
{\bf
($\sim$13.7 au given the Gaia parallax distance of 137 pc). 
Out towards $3\arcsec$ the contrast improves to $\Delta {\rm mag} = 7$.  
These $\Delta$mag limits rule out the presence of anything more luminous than approximately an M4V dwarf at $0\farcs1$ or M6V dwarf out towards $1\arcsec$.
}
The contrast curves are shown in Figure~\ref{fig:Speckle}.










\input{Table_CHIRON_RVs.tex} 



\input{Table_CHIRON_vs_SED.tex} 










%% CHIRON ruling out binary signals
Turning to spectroscopy, from the CHIRON data we derived RVs of TOI-1221 from the fitted line profiles of each spectrum, which were extracted using least-squares deconvolution (LSD) of the observed spectrum against synthetic templates \citep{Donati1997}. 
The RVs are listed in Table \ref{Tab:chiron_RVs}. Blended eclipsing binaries can produce spectral line profile variations as a function of orbital phase, but we find no evidence for additional stars or variable line profile shape in the spectra of TOI-1221.
{\bf The CHIRON RVs also show no large velocity variation across the 2-year baseline and wide phase coverage}.
%
With the relatively flat RVs, the $1\sigma$ and $3\sigma$ upper limits on the planet mass, given its period, are 1.1 M$_{\rm Jup}$ and 3.5 M$_{\rm Jup}$, respectively.  
While the RV measurements are not sensitive enough to rule out massive, outer planetary companions, these data provide evidence against additional stellar-mass components in the system with orbits near the period of the observed transit signals.
This is in line with the {\it Gaia} Renormalised Unit Weight Error (RUWE) measure of 1.11, which is consistent with expectations for a single star.  
%

%% ~13-80 MJ is a BD
%% > 80 MJ is an Mdwarf

% \notes{(The Saturn and Jupiter masses at 1 and 2 au do produce the observed slope, but the sinusoids are far higher frequency than matches the RV points which span $\sim2$ years.  I.e. the slopes only last 1/4 or 1/2 a year.  A 55 $M_J$ object (BD) at 14 au can produce the prolonged slope. A $0.24 M_\odot$ (M4V) makes the slope at 30 au, and is basically the first thing we could detect with Zorro.  With 3 points, there's also no guarantee that the ``slope" is not an alias of some high-frequency signal.)}

%
{\bf
While the RVs limit anything at $P~\sim 90$ days to planetary mass, a small, marginally significant RV slope exists ($0.13 \pm 0.053$ m s$^{-1}$ day$^{-1}$) that could indicate an additional massive object with a wider orbit.  
With only 3 data points, fitting any kind of model is problematic as the degrees of freedom are unacceptably low.
However, we can explore some limiting cases.
%
%
Let us restrict ourselves to simple circular edge-on orbits that could account for the observed slope.
The RVs exhibit this slope over their span of $\sim2$ years.  
A 2 $M_{\rm Jup}$ object on a 3 au orbit (5.2 year period) could produce the slope, but smaller orbits would have RV variations of too high a frequency.
%
On the other end of the scale, a $0.24 M_\odot$ star ($\sim$M4V) at 30 au (165 year period and angular separation of $0\farcs2$) could also produce the slope, but would be bright and separated enough to be detected in the Zorro image.
%
Any mass--period combination in between these scenarios can produce the observed slope while remaining undetected by Zorro. 
%
Photometrically, none of the objects in this range are  bright enough to have a significant impact on our transit fits. Even the brightest M-dwarf in that range would only cause a minor flux dilution.  It would affect our radius value by $<$1\%, smaller than our measured uncertainties.

Of course, actual RV curves depend strongly on orbital inclination, phase, and eccentricity, which are all unknown.  There is the additional possibility that the observed RV ``slope" is not in fact a true gradual slope, but undersampled aliasing of a signal with period shorter than the 2-year coverage.
%$g=14.75$ (dmag=4.25) gives 1\% radius error
}



%% Using TRICERATOPS for statistical validation.
As a final quantitative assessment of the planet's validity we used the \texttt{TRICERATOPS} (Tool for Rating
Interesting Candidate Exoplanets and Reliability Analysis of
Transits Originating from Proximate Stars) statistical validation package for {\it TESS} transits \citep{triceratops_code,triceratops_paper}.  
\texttt{TRICERATOPS} uses a Bayesian framework and was developed with {\it TESS} observations in mind.  It leverages the well-characterized stellar qualities in the {\it TESS} Input Catalog and specifically handles multiple blended stars in the large {\it TESS} apertures in a precise manner.
{\bf It calculates false positive probabilities by leveraging known information about background star rates and bound multiplicity priors.  It also uses provided contrast curves to refine its assessment.}

\texttt{TRICERATOPS} calculates an
% FPP
intrinsic false positive probability (FPP) which considers scenarios only involving absent or unresolved close neighbours,
% NFPP
as well as a nearby false positive probability (NFPP) which involves scenarios with nearby stars.
%
Based on comparisons to externally vetted TOIs, \texttt{TRICERATOPS} defines a planet candidate as validated if it achieves a FPP $<0.015$ and NFPP $<0.001$.
%
In the case of TOI-1221.01, we entered in the six detected {\it TESS} transits and the high-contrast limits placed by SOAR and Zorro imaging.  We calculate the values 
FPP $= 0.0014 \pm 0.0003$ 
and 
NFPP $= 0.0012 \pm 0.0004$.
%
The FPP statistic falls well below the \texttt{TRICERATOPS} validation threshold, and the NFPP straddles the threshold between "validated" and ``likely planet" designations.
{\bf
It is worth noting that {\tt TRICERATOPS} does not have a way to include RV acceleration constraints in its assessment.  Its findings, when RVs can provide additional information, are likely conservative.
}





In sections \ref{sSec:Transit_Fitting} and \ref{sSec:TTVs} we discuss the presence of transit timing variations (TTVs) in the observations.  This is additional qualitative evidence against the NEB hypothesis.  For the observed signals to be caused by a NEB, this NEB would have to exhibit TTVs and would therefore have to be a trinary (or more) system.  





%% Conclusion of section
{\bf
While TOI-1221.01 orbiting with the 91.7-day period passes all planetary validation checks, the data hint at the presence of another companion in the system.  The observations leave room for an another body out to roughly 30 au and up to about 0.24 $M_\odot$.  Such an companion does not pose photometric dilution issues, but may be implicated for inducing TTVs.}
%
With all these validation results taken together, we consider the practical false-positives ruled out.  From this point onward, we consider the transit events to be caused by a planet and fit the light curve following that assumption.  We will adopt the nomenclature of TOI-1221 b to refer to this planet moving forward.




==> Poisson_tests_for_background_stars.tex <==

To explore the innermost 0.1\arcsec that remains blended with the target, we can look to the local sky density of stars in the region to assess the probability of there being a source of a given magnitude blended with TOI-1221.  
To do so, we look again at the {\it Gaia} DR3 catalogue which is $\sim99\%$ complete down to a magnitude of g$\sim$20 \citep{Boubert_Everall_2020}. 
There are two issues to consider regarding unresolved stars, each with their own limiting magnitudes at which they might cause significant problems.  

%%
Firstly, an unresolved solo neighbour contributes to the total measured flux but does not dim during transit. As such, it dilutes the relative transit signal causing us to measure a shallower transit and infer a smaller planet radius than would be the case without it.  As an arbitrary cutoff, we have calculated the neighbour magnitude at which the dilution would cause a 1\% discrepancy in the extracted planetary radius.
This conservative limit occurs at $g=14.75$ and the 1\% error is smaller than the typical uncertainty we can place on the planetary radius.  Using the {\it Gaia} catalogue to assess the local density of stars brighter than this limit, we calculate an expectation rate at which such stars would appear in the small $r$=0.1\arcsec \ region left unresolved by the Gemini-S/Zorro image.  Assuming a Poisson distribution of stars, we determine the probability to be $1.5\times10^{-6}$, negligibly small, that at least one star falls in this region and has a magnitude problematic in the sense of signal dilution.

%%
Secondly, an unresolved neighbour could be a NEB, producing the observed transit signal while TOI-1221 itself remains unvarying.  The limiting problematic magnitude in this scenario is related to the point at which the NEB is too faint to produce the observed signal.  
%
%For instance, we expect an EB system to have a maximum flux drop of $\sim50\%$, corresponding to a full eclipse of equal-sized, equal-brightness bodies. 
%
Generally speaking, we expect the vast majority of EB events to display flux drops of <$50\%$ during eclipse.  This conservative limit corresponds to equal-mass binaries at a similar evolutionary stage at close to 90$^\circ$ inclination, even though the V-shaped eclipse light curves in such systems are morphologically distinct from planetary transits.  There are a few improbable scenarios that could produce planet-like transit shapes at depths >$50\%$ (e.g. EB of a sub-giant and an A star), but they would be very rare occurrences. 
%
The faintest NEB where a $50\%$ flux drop could still decrease the total combined flux by the $\sim$750 ppm measured by {\it TESS} is $g=17.63$.
%
Following the same Poisson process with the {\it Gaia} stars brighter than this limit leads to a probability of $8.6\times10^{-6}$ that a star capable of a sufficient EB flux drop is in the unconstrained region of TOI-1221. 
%
% -- from Hugh --
% “Equal mass binaries (50\% drop) don’t really produce transit-like light curves, but other scenarios (e.g. sub-giant + A star) do and can have depths >50\%.  But TRICERATOPS or VESPA should check for that.”
%
%
%%Note that this estimate does not factor in the probabilities that a given star \emph{is} an EB at all, or even consider that an EB flux drop of less than 50\% is far more likely, so the true probability will be substantially smaller and the limiting magnitude brighter.
%
Note that this estimate does not consider that shallower EB eclipses are far more likely to occur.  The true probability will be lower and the limiting magnitude brighter than calculated here. 
%%


==> Sections/Authors_MNRAS_final_order.tex <==
% The list of authors, and the short list which is used in the headers.
% If you need two or more lines of authors, add an extra line using \newauthor



\author[C. Mann et al.]{%
%
%
Christopher R. Mann\orcid{0000-0002-9312-0073},$^{1,2}$%
\thanks{E-mail: christopher.mann@umontreal.ca} %
%
David Lafrenière\orcid{0000-0002-6780-4252},$^{1,2}$
%
Diana Dragomir\orcid{0000-0003-2313-467X},$^{22}$
%
Samuel N. Quinn\orcid{0000-0002-8964-8377},$^{3}$ % CHIRON stuff
%
Thiam-Guan Tan\orcid{0000-0001-5603-6895},$^{4}$ % PEST obs
%
\and
%
Karen A.\ Collins\orcid{0000-0001-6588-9574},$^{3}$ % LCOGT - %karen.collins@cfa.harvard.edu
%
Steve B. Howell,$^{5}$ % Provided Gemini-S/Zorro speckle
%
Carl Ziegler,$^{6}$ %SOAR imaging 
%
Andrew W. Mann,$^{7}$ %SOAR imaging 
%
Keivan G. Stassun\orcid{0000-0002-3481-9052},$^{8}$ % SED analysis
%
\and
%
Martti~H.~Kristiansen\orcid{0000-0002-2607-138X},$^{9}$ % initial detection 
%
Hugh Osborn,$^{10,11}$ % Involved in initial assessment. Offered transit modelling + vetting
%
Tabetha Boyajian\orcid{0000-0001-9879-9313},$^{12}$ % provided first CHIRON spec measurement
%
Nora Eisner,$^{13}$ % provided first CHRION spec measurement
%
Coel Hellier,$^{14}$ %WASP-S modulation assessment
%
\and
%
George~R.~Ricker\orcid{0000-0003-2058-6662},$^{10}$ % TESS Architect
%
Roland~Vanderspek\orcid{0000-0001-6763-6562},$^{10}$ % TESS Architect
%
David~W.~Latham\orcid{0000-0001-9911-7388},$^{3}$ % TESS Architect
%
S.~Seager\orcid{0000-0002-6892-6948},$^{10,15,16}$ % TESS Architect
%
\and
%
Joshua~N.~Winn\orcid{0000-0002-4265-047X},$^{17}$ % TESS Architect
%
%
Jon~M.~Jenkins\orcid{0000-0002-4715-9460},$^{5}$ % TESS Architect
%
% Joel Villase{\~ n}or,$^{8}$ % POC
%
Brian~McLean\orcid{0000-0002-8058-643X},$^{18}$ % POC
%
Pamela~Rowden\orcid{0000-0002-4829-7101},$^{19}$ % POC
%
Guillermo~Torres\orcid{0000-0002-5286-0251},$^{3}$ % TSO
%
\and
%
Douglas A. Caldwell\orcid{0000-0003-1963-9616},$^{5,20}$ % SPOC
%
Kevin I.\ Collins\orcid{0000-0003-2781-3207},$^{21}$ %kcolli3@gmu.edu   
%
Richard P. Schwarz\orcid{0000-0001-8227-1020}$^{3}$ %rpschwarz@comcast.net
%
%
%
%
%
\vspace{0.3cm}
%
%
%
%
%
%
%
%
%
%
%
%
%
\\
% List of institutions
$^{1}$Université de Montréal, 1375 Ave. Thérèse-Lavoie-Roux, Montréal, QC H2V 0B3, Canada\\
$^{2}$Institute for Research on Exoplanets (\emph{iREx})\\
$^{3}$Center for Astrophysics \textbar \ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{4}$Perth Exoplanet Survey Telescope, Perth, Western Australia, Australia\\
$^{5}$NASA Ames Research Center, Moffett Field, CA\\
$^{6}$Department of Physics, Engineering and Astronomy, Stephen F. Austin State University, 1936 North St, Nacogdoches, TX 75962, USA\\
$^{7}$Department of Physics and Astronomy, The University of North Carolina at Chapel Hill, Chapel Hill, NC 27599-3255, USA\\
$^{8}$Department of Physics and Astronomy, Vanderbilt University, Nashville, TN 37235, USA\\
$^{9}$Brorfelde Observatory, Observator Gyldenkernes Vej 7, DK-4340 T\o{}ll\o{}se, Denmark\\
$^{10}$Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
$^{11}$Physikalisches Institut, University of Bern, Gesellsschaftstrasse 6, 3012 Bern, Switzerland\\
$^{12}$Louisiana State University 202 Nicholson Hall Baton Rouge, LA 70803, USA\\
$^{13}$Sub-department of Astrophysics, University of Oxford, Keble Rd, Oxford, United Kingdom\\
$^{14}$Astrophysics Group, Keele University, Staffordshire ST5 5BG, U.K.\\
$^{15}$Department of Earth, Atmospheric and Planetary Sciences, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
$^{16}$Department of Aeronautics and Astronautics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
$^{17}$Department of Astrophysical Sciences, Princeton University, 4 Ivy Lane, Princeton, NJ 08544, USA\\
$^{18}$Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD, 21218, USA\\
$^{19}$Royal Astronomical Society, Burlington House, Piccadilly, London W1J 0BQ, UK\\
$^{20}$SETI Institute\\
$^{21}$George Mason University, 4400 University Drive, Fairfax, VA, 22030 USA\\
$^{22}$Department of Physics and Astronomy, University of New Mexico, 1919 Lomas Blvd NE Albuquerque, NM, 87131, USA\\
%
%
%
%
%
% \cmc{$^{**}$}\cmc{Unknown affiliation}
}

==> Table_Derived_parameters.tex <==
\begin{table}
\caption{Derived parameters}
\centering
\label{Tab:Derived_params}
\def\arraystretch{1.5}%  1 is the default, change whatever you need
\begin{tabular}{ccc}
\hline
Parameter &  Value  &  Units    \\
\hline

$a/R_{\star}$          & $83.7^{+4.7}_{-4.0}$      & --   \\
$i$              & $89.75^{+0.16}_{-0.08}$   & deg  \\
$e$              & $<0.21$                   & --   \\
$\omega^\prime$  & $108^{+37}_{-43}$         & deg  \\
$u_{\rm 1:TESS}$ & $0.35^{+0.02}_{-0.02}$    &  --  \\
$u_{\rm 2:TESS}$ & $0.16^{+0.02}_{-0.01}$    &  --  \\
$u_{\rm 1:LCOGT}$& $0.30^{+0.02}_{-0.02}$    &  --  \\
$u_{\rm 2:LCOGT}$& $0.20^{+0.01}_{-0.02}$    &  --  \\

\hline
\end{tabular}
\raggedright
\newline\noindent 
\textbf{Note.} The derived posterior on eccentricity places a 68\% confidence upper limit.  The parameter $\omega^\prime$ is used as a proxy for the argument of pericentre ($\omega$).  When eccentricity is low, the light curve shape is largely insensitive to whether the transit occurs before or after pericentre passage.  This causes a strongly bimodal distribution in $\omega$.  We define $\omega^\prime$ as the absolute angle between the line of sight and pericentre passage, which collapses to a unimodal posterior and is easier to present in a table.
\end{table}


==> Table_Fitted_parameters.tex <==
\begin{table}
\caption{Directly fitted parameters}
\centering
\label{Tab:fitted_params}
\def\arraystretch{1.5}%  1 is the default, change whatever you need
\begin{tabular}{cccc}
\hline
Parameter &  Value  &  Units   &  Prior   \\
\hline

$P$           & $91.68278^{+0.00032}_{-0.00041}$   & days  &  -- \\
$T_0$         & $2458404.1791^{+0.0035}_{-0.0030}$ & BJD$_{\rm TDB}$ &  --  \\
$R_{\rm p}/R_{\star}$& $0.02679^{+0.00067}_{-0.00056}$    &  --  &  $\mathcal{U}[0.0,0.05]$  \\
$b$   & $0.25^{+0.22}_{-0.14}$             &  --  &  $\mathcal{U}[0.0,1.027]$  \\
$q_{\rm 1:TESS}$ & $0.26^{+0.02}_{-0.01}$          &  --  &  $\mathcal{N}(0.264,0.02)$     \\
$q_{\rm 2:TESS}$ & $0.34^{+0.01}_{-0.02}$          &  --  &  $\mathcal{N}(0.334,0.02)$     \\
$q_{\rm 1:LCOGT}$& $0.25^{+0.02}_{-0.03}$          &  --  &    $\mathcal{N}(0.250,0.02)$   \\
$q_{\rm 2:LCOGT}$& $0.30^{+0.02}_{-0.02}$          &  --  &    $\mathcal{N}(0.301,0.02)$   \\
$\esinw$      & $0.00^{+0.16}_{-0.26}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
$\ecosw$      & $0.01^{+0.40}_{-0.39}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
$\rho_{\star}$& $1320^{+220}_{-190}$               &  kg m$^{-3}$ & $\mathcal{N}(1349, 296)$  \\
%
%
%
$T_{\#0:TESS}$&$2458404.1844^{+0.0060}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458404.1850, 0.02)$  \\
$T_{\#1:TESS}$&$2458495.8474^{+0.0075}_{-0.0048}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458495.8681, 0.02)$  \\
$T_{\#2:TESS}$&$2458587.5401^{+0.0061}_{-0.0087}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458587.5511, 0.02)$  \\
$T_{\#3:TESS}$&$2458679.2361^{+0.0056}_{-0.0056}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458679.2342, 0.02)$  \\
$T_{\#8:TESS}$&$2459137.6494^{+0.0043}_{-0.0061}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459137.6494, 0.02)$  \\
$T_{\#9:TESS}$&$2459229.3342^{+0.0067}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459229.3325, 0.02)$  \\
$T_{\#12:LCOGT}$&$2459504.3456^{+0.0054}_{-0.0047}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459504.3690, 0.02)$  \\
$T_{\#14:LCOGT}$&$2459687.7466^{+0.0044}_{-0.0044}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459687.7500, 0.02)$  \\

\hline
\end{tabular}
\raggedright
% \newline\noindent 
\textbf{Note.} Priors were of two varieties: Uniform over a given interval, $\mathcal{U}[a,b]$, and normal with stated mean and standard deviation, $\mathcal{N}(\mu,\sigma)$.  Gaussian process parameters are omitted here for readability because they always fit to amplitudes at least an order of magnitude smaller than the transit depth.

\end{table}


==> Table_all_params.tex <==
\begin{table*}
\caption{Directly fitted parameters}
\centering
\label{Tab:all_params}
\def\arraystretch{1.5}%  1 is the default, change whatever you need
\begin{tabular}{llccc}
\hline
Parameter & Description & Value  &  Units   &  Prior   \\
\hline

% \smallskip\\
\multicolumn{2}{l}{Target Parameters:}&\smallskip\\



~~~~$P$\dotfill &  Period\dotfill    & $91.68278^{+0.00032}_{-0.00041}$   & days  &  -- \\
~~~~$T_0$\dotfill &  Epoch reference\dotfill         & $2458404.1791^{+0.0035}_{-0.0030}$ & BJD$_{\rm TDB}$ &  --  \\
~~~~$R_{\rm p}/R_{\star}$\dotfill&  Planet radius in stellar radii\dotfill & $0.02679^{+0.00067}_{-0.00056}$    &  --  &  $\mathcal{U}[0.0,0.05]$  \\
~~~~$b$\dotfill &  Impact parameter\dotfill   & $0.25^{+0.22}_{-0.14}$             &  --  &  $\mathcal{U}[0.0,1.027]$  \\

~~~~$\esinw$\dotfill   &  $e,\omega$ Parameterization \dotfill    & $0.00^{+0.16}_{-0.26}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
~~~~$\ecosw$\dotfill  &  $e,\omega$ Parameterization\dotfill     & $0.01^{+0.40}_{-0.39}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
~~~~$\rho_{\star}$\dotfill&  Stellar density\dotfill & $1320^{+220}_{-190}$               &  kg m$^{-3}$ & $\mathcal{N}(1349, 296)$  \\
~~~~$T_{\#0:TESS}$\dotfill&  Epoch 0 transit midpoint \dotfill &$2458404.1844^{+0.0060}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458404.1850, 0.02)$  \\
~~~~$T_{\#1:TESS}$\dotfill&  Epoch 1 transit midpoint\dotfill &$2458495.8474^{+0.0075}_{-0.0048}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458495.8681, 0.02)$  \\
~~~~$T_{\#2:TESS}$\dotfill&  Epoch 2 transit midpoint\dotfill &$2458587.5401^{+0.0061}_{-0.0087}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458587.5511, 0.02)$  \\
~~~~$T_{\#3:TESS}$\dotfill&  Epoch 3 transit midpoint\dotfill &$2458679.2361^{+0.0056}_{-0.0056}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458679.2342, 0.02)$  \\
~~~~$T_{\#8:TESS}$\dotfill&  Epoch 8 transit midpoint\dotfill &$2459137.6494^{+0.0043}_{-0.0061}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459137.6494, 0.02)$  \\
~~~~$T_{\#9:TESS}$\dotfill&  Epoch 9 transit midpoint\dotfill &$2459229.3342^{+0.0067}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459229.3325, 0.02)$  \\
~~~~$T_{\#12:LCOGT}$\dotfill&  Epoch 12 transit midpoint\dotfill &$2459504.3456^{+0.0054}_{-0.0047}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459504.3690, 0.02)$  \\
~~~~$T_{\#14:LCOGT}$\dotfill&  Epoch 14 transit midpoint \dotfill &$2459687.7466^{+0.0044}_{-0.0044}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459687.7500, 0.02)$  \\
%
%
% \smallskip\\
\multicolumn{2}{l}{Telescope Parameters:}&\smallskip\\
%
%
~~~~$q_{\rm 1:TESS}$\dotfill&  Quadratic limb darkening coefficient\dotfill  & $0.26^{+0.02}_{-0.01}$          &  --  &  $\mathcal{N}(0.264,0.02)$     \\
~~~~$q_{\rm 2:TESS}$\dotfill&  Quadratic limb darkening coefficient\dotfill  & $0.34^{+0.01}_{-0.02}$          &  --  &  $\mathcal{N}(0.334,0.02)$     \\
~~~~$q_{\rm 1:LCOGT}$\dotfill&  Quadratic limb darkening coefficient\dotfill & $0.25^{+0.02}_{-0.03}$          &  --  &    $\mathcal{N}(0.250,0.02)$   \\
~~~~$q_{\rm 2:LCOGT}$\dotfill&  Quadratic limb darkening coefficient\dotfill & $0.30^{+0.02}_{-0.02}$          &  --  &    $\mathcal{N}(0.301,0.02)$   \\

% \smallskip\\
\multicolumn{2}{l}{Placeholder:}&\smallskip\\
%

~~~~$a/R_{\star}$\dotfill  & Semi-major axis in stellar radii \dotfill   & $83.7^{+4.7}_{-4.0}$      & --  &  --  \\
~~~~$i$\dotfill            & Inclination \dotfill   & $89.75^{+0.16}_{-0.08}$   & deg &  -- \\
~~~~$e$\dotfill            & Eccentricity \dotfill   & $<0.21$                   & --  &  -- \\
~~~~$\omega^\prime$\dotfill & Modified argument of pericentre$^{2}$ \dotfill  & $108^{+37}_{-43}$         & deg &  -- \\
~~~~$u_{\rm 1:TESS}$\dotfill& Quadratic limb darkening coefficient \dotfill  & $0.35^{+0.02}_{-0.02}$    &  -- &  -- \\
~~~~$u_{\rm 2:TESS}$\dotfill& Quadratic limb darkening coefficient \dotfill  & $0.16^{+0.02}_{-0.01}$    &  -- &  -- \\
~~~~$u_{\rm 1:LCOGT}$\dotfill& Quadratic limb darkening coefficient \dotfill & $0.30^{+0.02}_{-0.02}$    &  -- &  -- \\
~~~~$u_{\rm 2:LCOGT}$\dotfill& Quadratic limb darkening coefficient \dotfill & $0.20^{+0.01}_{-0.02}$    &  -- &  -- \\

~~~~ $R_p$ \dotfill & Planet radius \dotfill & $X^{+Y}_{-Z}$    & $R_\oplus$ &  -- \\
~~~~ $M_p$ \dotfill & Planet mass$^{3}$ \dotfill & $X^{+Y}_{-Z}$    & $M_\oplus$ &  -- \\
~~~~ $S_p$ \dotfill & Insolation \dotfill & $X^{+Y}_{-Z}$    &  $S_\oplus$ &  -- \\
~~~~ $T_{\rm eq}$ \dotfill & Equilibrium temperature \dotfill & $X^{+Y}_{-Z}$    &  K &  -- \\

~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\


\hline
\end{tabular}
% \raggedright
\newline%\noindent 
% \vspace{0.2cm}

\tablenotetext{}{\textbf{Note.} 
Directly fitted parameters include a prior description.
Priors were of two varieties: Uniform over a given interval, $\mathcal{U}[a,b]$, and normal with stated mean and standard deviation, $\mathcal{N}(\mu,\sigma)$.
%
If no prior is specified, the quantity was calculated from fitted parameters.
%
Gaussian process parameters are omitted here for readability because they always fit to amplitudes at least an order of magnitude smaller than the transit depth.
}

\tablenotetext{2}{
When eccentricity is low the light curve shape is insensitive to whether the transit occurs before or after pericentre passage. We define $\omega^\prime$ as the absolute angle between the line of sight and pericentre passage. This collapses $\omega$'s strongly bimodal distribution to a unimodal posterior and is easier to present in a table.
}

\end{table*}


==> Table_all_params_deluxtable.tex <==
\startlongtable
\begin{deluxetable*}{llccc}
\tablecaption{\cmc{Table Caption}}
%
\tablehead{\colhead{~~~Parameter} & \colhead{Description} & \colhead{Value} & \colhead{Units}  & \colhead{Prior}}
\startdata
%
%
% Parameter & Description & Value  &  Units   &  Prior   \\
% \hline
%
% \smallskip\\
\multicolumn{5}{l}{Target Parameters:}&\smallskip\\
%
%
%
~~~~$P$\dotfill &  Period\dotfill    & $91.68278^{+0.00032}_{-0.00041}$   & days  &  -- \\
~~~~$T_0$\dotfill &  Epoch reference\dotfill         & $2458404.1791^{+0.0035}_{-0.0030}$ & BJD$_{\rm TDB}$ &  --  \\
~~~~$R_{\rm p}/R_{\star}$\dotfill&  Planet radius in stellar radii\dotfill & $0.02679^{+0.00067}_{-0.00056}$    &  --  &  $\mathcal{U}[0.0,0.05]$  \\
~~~~$b$\dotfill &  Impact parameter\dotfill   & $0.25^{+0.22}_{-0.14}$             &  --  &  $\mathcal{U}[0.0,1.027]$  \\
%%
~~~~$\esinw$\dotfill   &  $e,\omega$ Parameterization \dotfill    & $0.00^{+0.16}_{-0.26}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
~~~~$\ecosw$\dotfill  &  $e,\omega$ Parameterization\dotfill     & $0.01^{+0.40}_{-0.39}$           & -- & $\mathcal{U}[-1.0,1.0]$   \\
~~~~$\rho_{\star}$\dotfill&  Stellar density\dotfill & $1320^{+220}_{-190}$               &  kg m$^{-3}$ & $\mathcal{N}(1349, 296)$  \\
~~~~$T_{\#0:TESS}$\dotfill&  Epoch 0 transit midpoint \dotfill &$2458404.1844^{+0.0060}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458404.1850, 0.02)$  \\
~~~~$T_{\#1:TESS}$\dotfill&  Epoch 1 transit midpoint\dotfill &$2458495.8474^{+0.0075}_{-0.0048}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458495.8681, 0.02)$  \\
~~~~$T_{\#2:TESS}$\dotfill&  Epoch 2 transit midpoint\dotfill &$2458587.5401^{+0.0061}_{-0.0087}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458587.5511, 0.02)$  \\
~~~~$T_{\#3:TESS}$\dotfill&  Epoch 3 transit midpoint\dotfill &$2458679.2361^{+0.0056}_{-0.0056}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2458679.2342, 0.02)$  \\
~~~~$T_{\#8:TESS}$\dotfill&  Epoch 8 transit midpoint\dotfill &$2459137.6494^{+0.0043}_{-0.0061}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459137.6494, 0.02)$  \\
~~~~$T_{\#9:TESS}$\dotfill&  Epoch 9 transit midpoint\dotfill &$2459229.3342^{+0.0067}_{-0.0051}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459229.3325, 0.02)$  \\
~~~~$T_{\#12:LCOGT}$\dotfill&  Epoch 12 transit midpoint\dotfill &$2459504.3456^{+0.0054}_{-0.0047}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459504.3690, 0.02)$  \\
~~~~$T_{\#14:LCOGT}$\dotfill&  Epoch 14 transit midpoint \dotfill &$2459687.7466^{+0.0044}_{-0.0044}$ &BJD$_{\rm TDB}$& $\mathcal{N}(2459687.7500, 0.02)$  \\
%%
%%
%% \smallskip\\
\multicolumn{2}{l}{Telescope Parameters:}&\smallskip\\
%%
%%
~~~~$q_{\rm 1:TESS}$\dotfill&  Quadratic limb darkening coefficient\dotfill  & $0.26^{+0.02}_{-0.01}$          &  --  &  $\mathcal{N}(0.264,0.02)$     \\
~~~~$q_{\rm 2:TESS}$\dotfill&  Quadratic limb darkening coefficient\dotfill  & $0.34^{+0.01}_{-0.02}$          &  --  &  $\mathcal{N}(0.334,0.02)$     \\
~~~~$q_{\rm 1:LCOGT}$\dotfill&  Quadratic limb darkening coefficient\dotfill & $0.25^{+0.02}_{-0.03}$          &  --  &    $\mathcal{N}(0.250,0.02)$   \\
~~~~$q_{\rm 2:LCOGT}$\dotfill&  Quadratic limb darkening coefficient\dotfill & $0.30^{+0.02}_{-0.02}$          &  --  &    $\mathcal{N}(0.301,0.02)$   \\
%%
% \smallskip\\
\multicolumn{2}{l}{Placeholder:}&\smallskip\\
%
%%%
~~~~$a/R_{\star}$\dotfill  & Semi-major axis in stellar radii \dotfill   & $83.7^{+4.7}_{-4.0}$      & --  &  --  \\
~~~~$i$\dotfill            & Inclination \dotfill   & $89.75^{+0.16}_{-0.08}$   & deg &  -- \\
~~~~$e$\dotfill            & Eccentricity \dotfill   & $<0.21$                   & --  &  -- \\
~~~~$\omega^\prime$\dotfill & Modified argument of pericentre$^{2}$ \dotfill  & $108^{+37}_{-43}$         & deg &  -- \\
~~~~$u_{\rm 1:TESS}$\dotfill& Quadratic limb darkening coefficient \dotfill  & $0.35^{+0.02}_{-0.02}$    &  -- &  -- \\
~~~~$u_{\rm 2:TESS}$\dotfill& Quadratic limb darkening coefficient \dotfill  & $0.16^{+0.02}_{-0.01}$    &  -- &  -- \\
~~~~$u_{\rm 1:LCOGT}$\dotfill& Quadratic limb darkening coefficient \dotfill & $0.30^{+0.02}_{-0.02}$    &  -- &  -- \\
~~~~$u_{\rm 2:LCOGT}$\dotfill& Quadratic limb darkening coefficient \dotfill & $0.20^{+0.01}_{-0.02}$    &  -- &  -- \\
%%
~~~~ $R_p$ \dotfill & Planet radius \dotfill & $X^{+Y}_{-Z}$    & $R_\oplus$ &  -- \\
~~~~ $M_p$ \dotfill & Planet mass$^{3}$ \dotfill & $X^{+Y}_{-Z}$    & $M_\oplus$ &  -- \\
~~~~ $S_p$ \dotfill & Insolation \dotfill & $X^{+Y}_{-Z}$    &  $S_\oplus$ &  -- \\
~~~~ $T_{\rm eq}$ \dotfill & Equilibrium temperature \dotfill & $X^{+Y}_{-Z}$    &  K &  -- \\
%%
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &  -- &  -- \\
%
\enddata
\label{tab:full_results} 
%
\tablenotetext{}{\textbf{Note.} 
Directly fitted parameters include a prior description.
Priors were of two varieties: Uniform over a given interval, $\mathcal{U}[a,b]$, and normal with stated mean and standard deviation, $\mathcal{N}(\mu,\sigma)$.
%
If no prior is specified, the quantity was calculated from fitted parameters.
%
Gaussian process parameters are omitted here for readability because they always fit to amplitudes at least an order of magnitude smaller than the transit depth.
}
%
\tablenotetext{2}{
When eccentricity is low the light curve shape is insensitive to whether the transit occurs before or after pericentre passage. We define $\omega^\prime$ as the absolute angle between the line of sight and pericentre passage. This collapses $\omega$'s strongly bimodal distribution to a unimodal posterior and is easier to present in a table.
}
%
\end{deluxetable*}


==> Table_all_params_deluxtable3_didntwork.tex <==
\startlongtable
\begin{deluxetable*}{llccc}
% \tablecaption{\cmc{Table Caption}}
%
\tablehead{\colhead{~~~Parameter} & \colhead{Description (Units)} & \multicolumn{2}{c}{Values} & \colhead{Prior}}
\startdata
%
%
% Parameter & Description & Value  &  Units   &  Prior   \\
% \hline
%
% \smallskip\\
\multicolumn{2}{l}{Target Parameters:}  \\
%
%
%
~~~~$P$\dotfill &  Period$^{a}$ (days)\dotfill    & $91.68278^{+0.00032}_{-0.00041}$  &    &  -- \\
~~~~$T_0$\dotfill &  Epoch reference$^{a}$ (BJD$_{\rm TDB}$)\dotfill         & $2458404.1791^{+0.0035}_{-0.0030}$ &  &  --  \\
~~~~$R_{\rm p}/R_{\star}$\dotfill&  Planet radius in stellar radii\dotfill & $0.02679^{+0.00067}_{-0.00056}$    & &  $\mathcal{U}[0.0,0.05]$  \\
~~~~$b$\dotfill &  Impact parameter\dotfill   & $0.25^{+0.22}_{-0.14}$        &   &  $\mathcal{U}[0.0,1.027]$  \\
%%
%
%
~~~~$a/R_{\star}$\dotfill  & Semi-major axis in stellar radii \dotfill   & $83.7^{+4.7}_{-4.0}$     &  &  --  \\
~~~~$i$\dotfill            & Inclination (deg)\dotfill   & $89.75^{+0.16}_{-0.08}$  &  &  -- \\
~~~~$e$\dotfill            & Eccentricity \dotfill   & $<0.21$                   &   &  -- \\
~~~~$\omega^\prime$\dotfill & Modified argument of pericentre$^{b}$ (deg) \dotfill  & $108^{+37}_{-43}$   &   &   -- \\
~~~~$\esinw$\dotfill   &  $e,\omega$ parameterization \dotfill    & $0.00^{+0.16}_{-0.26}$      &  & $\mathcal{U}[-1.0,1.0]$   \\
~~~~$\ecosw$\dotfill  &  $e,\omega$ parameterization\dotfill     & $0.01^{+0.40}_{-0.39}$      &  & $\mathcal{U}[-1.0,1.0]$   \\
%%
~~~~$R_p$ \dotfill & Planet radius ($R_\oplus$)\dotfill & $2.91^{+0.13}_{-0.12}$   &  &   -- \\
~~~~$\rho_p$ \dotfill & Planet density$^{f}$ (g cm$^{-3}$) \dotfill & $2.6 \pm 0.2$  &  &   -- \\
~~~~$M_p$ \dotfill & Planet mass$^{f}$ ($M_\oplus$)\dotfill & $11.6\pm1.7$   &  &  -- \\
~~~~$\log g_p$ \dotfill & Surface Gravity$^{f}$ ($g_p$ given in cm s$^{-2}$) \dotfill & $3.12 \pm 0.08$   & &   -- \\
~~~~$K$ \dotfill & RV semi-amplitude$^{f}$ \dotfill & 1.62 \pm 0.25   & &   -- \\
~~~~$S_p$ \dotfill & Insolation$^{e}$ ($S_\oplus$)\dotfill & $6.06^{+0.85}_{-0.77}$    &  &   -- \\
~~~~$T_{14}$ \dotfill & Transit duration (hours) \dotfill & $8.12^{+1.01}_{-1.14}$    & &   -- \\
~~~~$a$ \dotfill & Semi-major axis (au) \dotfill & $0.387^{+0.026}_{-0.023}$    &  &  -- \\
~~~~$\delta$ \dotfill &Transit depth $(R_p/R_\star)^2$ \dotfill & $0.00072^{+0.00004}_{-0.00003}$    & &   -- \\
~~~~$T_{\rm eq}$ \dotfill & Equilibrium temperature$^{g}$ (K)\dotfill & $440\pm60$    &  &   -- \\
%
%
%
%
%
~~~~$\rho_{\star}$\dotfill&  Stellar density (kg m$^{-3}$)\dotfill & $1320^{+220}_{-190}$               &   & $\mathcal{N}(1349, 296)$  \\
~~~~$T_{\#0:TESS}$\dotfill&  Epoch 0 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2458404.1844^{+0.0060}_{-0.0051}$ & & $\mathcal{N}(2458404.1850, 0.02)$  \\
~~~~$T_{\#1:TESS}$\dotfill&  Epoch 1 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2458495.8474^{+0.0075}_{-0.0048}$ & & $\mathcal{N}(2458495.8681, 0.02)$  \\
~~~~$T_{\#2:TESS}$\dotfill&  Epoch 2 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2458587.5401^{+0.0061}_{-0.0087}$ & & $\mathcal{N}(2458587.5511, 0.02)$  \\
~~~~$T_{\#3:TESS}$\dotfill&  Epoch 3 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2458679.2361^{+0.0056}_{-0.0056}$ & & $\mathcal{N}(2458679.2342, 0.02)$  \\
~~~~$T_{\#8:TESS}$\dotfill&  Epoch 8 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2459137.6494^{+0.0043}_{-0.0061}$ & & $\mathcal{N}(2459137.6494, 0.02)$  \\
~~~~$T_{\#9:TESS}$\dotfill&  Epoch 9 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2459229.3342^{+0.0067}_{-0.0051}$ & & $\mathcal{N}(2459229.3325, 0.02)$  \\
~~~~$T_{\#12:LCOGT}$\dotfill&  Epoch 12 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2459504.3456^{+0.0054}_{-0.0047}$ & & $\mathcal{N}(2459504.3690, 0.02)$  \\
~~~~$T_{\#14:LCOGT}$\dotfill&  Epoch 14 transit midpoint (BJD$_{\rm TDB}$)\dotfill &$2459687.7466^{+0.0044}_{-0.0044}$ & & $\mathcal{N}(2459687.7500, 0.02)$ \smallskip \\
%%
%%
\smallskip\\\multicolumn{2}{l}{Telescope-specific parameters}&TESS&LCOGT\smallskip\\
% \multicolumn{4}{l}{Telescope-specific Parameters:} \smallskip\\
%%
%%
%
%
~~~~$q_1$\dotfill &linear limb-darkening coeff \dotfill &$0.0\pm0.0$ & $0.0\pm0.0$ & $\mathcal{N}(0.264,0.02)$  \\
%
%
%
%
%
% ~~~~$q_{\rm 1:TESS}$\dotfill&  Quadratic limb darkening coefficient$^{c}$\dotfill  & $0.26^{+0.02}_{-0.01}$          &  $\mathcal{N}(0.264,0.02)$     \\
% ~~~~$q_{\rm 2:TESS}$\dotfill&  Quadratic limb darkening coefficient$^{c}$\dotfill  & $0.34^{+0.01}_{-0.02}$          &  $\mathcal{N}(0.334,0.02)$     \\
% ~~~~$q_{\rm 1:LCOGT}$\dotfill&  Quadratic limb darkening coefficient$^{c}$\dotfill & $0.25^{+0.02}_{-0.03}$           &    $\mathcal{N}(0.250,0.02)$   \\
% ~~~~$q_{\rm 2:LCOGT}$\dotfill&  Quadratic limb darkening coefficient$^{c}$\dotfill & $0.30^{+0.02}_{-0.02}$            &    $\mathcal{N}(0.301,0.02)$   \\
% ~~~~$u_{\rm 1:TESS}$\dotfill& Quadratic limb darkening coefficient$^{c}$ \dotfill  & $0.35^{+0.02}_{-0.02}$    &  -- \\
% ~~~~$u_{\rm 2:TESS}$\dotfill& Quadratic limb darkening coefficient$^{c}$ \dotfill  & $0.16^{+0.02}_{-0.01}$   &  -- \\
% ~~~~$u_{\rm 1:LCOGT}$\dotfill& Quadratic limb darkening coefficient$^{c}$ \dotfill & $0.30^{+0.02}_{-0.02}$    &  -- \\
% ~~~~$u_{\rm 2:LCOGT}$\dotfill& Quadratic limb darkening coefficient$^{c}$ \dotfill & $0.20^{+0.01}_{-0.02}$    &  -- \\
% %%
% %
% %
% ~~~~$\mu_{\rm TESS}$ \dotfill & TESS relative flux offset \dotfill & $-0.00011 \pm 0.00001$   &  $\mathcal{N}(0.0,0.1)$ \\
% ~~~~$\mu_{\rm LCOGT}$ \dotfill & LCOGT relative flux offset \dotfill & $0.00003 \pm 0.00004$   &  $\mathcal{N}(0.0,0.1)$ \\
% %
% %
% ~~~~$\sigma_{GP:TESS}$ \dotfill & GP amplitude (ppm) \dotfill & $<0.132$   &   $\mathcal{L}[10^{-6},10^2]$ \\
% ~~~~$\rho_{GP:TESS}$ \dotfill & GP time-scale of Matern part\dotfill & $<0.725$   &   $\mathcal{L}[10^{-6},10^2]$ \\
% ~~~~$\tau_{GP:TESS}$ \dotfill & GP time-scale of exponential part \dotfill & $<0.013$   &   $\mathcal{L}[10^{-6},10^2]$ \\
% ~~~~$\sigma_{GP:LCOGT}$ \dotfill & GP amplitude (ppm) \dotfill & $<0.175$   &   $\mathcal{L}[10^{-6},10^2]$ \\
% ~~~~$\rho_{GP:LCOGT}$ \dotfill & GP time-scale of Matern part\dotfill & $<0.486$   &   $\mathcal{L}[10^{-6},10^2]$ \\
% ~~~~$\tau_{GP:LCOGT}$ \dotfill & GP time-scale of exponential part \dotfill & $<0.148$  &   $\mathcal{L}[10^{-6},10^2]$ \\
%
%
%
%
%
%
%
% \smallskip\\
% \multicolumn{4}{l}{Placeholder:}\smallskip\\
%
%%%
%%
% ~~~~ Name \dotfill & Description \dotfill & $X^{+Y}_{-Z}$    &   -- \\
%
\enddata
\label{tab:full_results} 
%
\tablenotetext{}{%
Directly fitted parameters include a prior description.
Priors are of three varieties: Uniform over a given interval, $\mathcal{U}[a,b]$, normal with stated mean and standard deviation, $\mathcal{N}(\mu,\sigma)$, or log-uniform over a stated range, $\mathcal{L}[a,b]$.
%
If no prior is specified, the quantity was calculated from other parameters.
%
% \cmc{Gaussian process parameters are omitted here for readability because they always fit to amplitudes at least an order of magnitude smaller than the transit depth.}
}
%
\tablenotetext{a}{
$P$ and $T_0$ are determined as the best-fit linear ephemeris around which the individual transit timings vary.
}
%
\tablenotetext{b}{
When eccentricity is low the light curve shape is insensitive to whether the transit occurs before or after pericentre passage. We define $\omega^\prime$ as the absolute angle between the line of sight and pericentre passage. This collapses $\omega$'s strongly bimodal distribution to a unimodal posterior and is easier to present in a written table.  $\omega$ has peaks at $198^\circ$ and $342^\circ$.
}
%
\tablenotetext{c}{ For descriptions of the different parameterizations $\{u_1,u_2\}$ vs. $\{q_1,q_2\}$ see definitions and discussion in \citet{Kipping_2013}. \cmc{(CHECK)} }
%
\tablenotetext{e}{ Insolation level assumes an orbital distance of $r=a$. }
%
\tablenotetext{f}{ 
\cmc{The density estimate of $\rho_p = 2.6 \pm 0.2$ g cm$^{-3}$ was derived from the figures ??? of Luque \& Pallé 2022 for sub-Neptune objects and was used to calculate mass-related quantities ($M_p,\log g_p$, and $K$).}}
%
\tablenotetext{g}{ \cmc{Assuming an albedo of XXXX and perfect thermal redistribution.} }
%
\end{deluxetable*}


